Modelling of nonlinear wave scattering in a delaminated elastic bar

Integrity of layered structures, extensively used in modern industry, strongly depends on the quality of their interfaces; poor adhesion or delamination can lead to a failure of the structure. Can nonlinear waves help us to control the quality of layered structures? In this paper we numerically model the dynamics of a long longitudinal strain solitary wave in a split, symmetric layered bar. The recently developed analytical approach, based on matching two asymptotic multiple-scales expansions and the integrability theory of the KdV equation by the Inverse Scattering Transform, is used to develop an effective semi-analytical numerical approach for these types of problems. We also employ a direct finite-difference method and compare the numerical results with each other, and with the analytical predictions. The numerical modelling confirms that delamination causes fission of an incident solitary wave and, thus, can be used to detect the defect.

==> title.tex <==
\begin{titlepage}
\begin{center}
{\Huge \textbf{Modelling of nonlinear wave scattering in a delaminated elastic bar}} \\[2.5em]
{\Large K. R. Khusnutdinova, M. R. Tranter} \\[2.5em]
{\Large Matthew Tranter} \\[1em]
{\Large Department of Mathematical Sciences, Loughborough University, Loughborough, LE11 3TU, United Kingdom} \\[2.5em]
{\Large Corresponding Author: K.Khusnutdinova@lboro.ac.uk}
\end{center}
\end{titlepage}
